A transition from river networks to scale-free networks

A spatial network is constructed on a two dimensional space where the nodes are geometrical points located at randomly distributed positions which are labeled sequentially in increasing order of one of their co-ordinates. Starting with $N$ such points the network is grown by including them one by one according to the serial number into the growing network. The $t$-th point is attached to the $i$-th node of the network using the probability: $\pi_i(t) \sim k_i(t)\ell_{ti}^{\alpha}$ where $k_i(t)$ is the degree of the $i$-th node and $\ell_{ti}$ is the Euclidean distance between the points $t$ and $i$. Here $\alpha$ is a continuously tunable parameter and while for $\alpha=0$ one gets the simple Barab\'asi-Albert network, the case for $\alpha \to -\infty$ corresponds to the spatially continuous version of the well known Scheidegger's river network problem. The modulating parameter $\alpha$ is tuned to study the transition between the two different critical behaviors at a specific value $\alpha_c$ which we numerically estimate to be -2.

==> list_of_changes <==


    List of Changes:

    We agree all the points raised by the referees and made
    the suitable changes as follows:

    General
    -------

    The full name of the first author is Anjan Kumar Nandi.
    The middle name was dropped. We now revise it as:
    A. K. Nandi.

    On the first referee's report
    -----------------------------

    1. We agree fully. They were our mistakes. $\alpha_c$ is
       indeed equal to -2. We have made the necessary changes
       at all places.
    2. Similarly $\alpha_c(N)$ values are also negative. They
       are also corrected.
    3. We agree. The Fig. 3 now shows the required data plot
       with the fit as adviced. Other two figures are therefore
       renamed as Fig. 4 and Fig. 5 and text has been revised
       accordingly.
    4. We agree. We have plotted the variation of the scaling
       exponents $\nu_k$, $\mu_k$ and $\gamma_k$ with $\alpha$
       in Fig. 4(a).

    5. This is a very general result and therefore we referred
       the book in ref. [5] in this context.

    6. The suggested references have been added in [21] and [22].

    On the second referee's report
    -----------------------------

    1. We agree. The required changes have been made in the abstract.

    Starting with $N$ such points the network is grown by including them one 
    by one according to the serial number into the growing network. The $t$-th 
    point is attached to the $i$-th node of the network using the probability: 
    $\pi_i(t) \sim k_i(t)\ell_{ti}^{\alpha}$ where $k_i(t)$ is the degree of 
    the $i$-th node and $\ell_{ti}$ is the Euclidean distance between the 
    points $t$ and $i$.

    2. We agree. We revise this portion in the following way:

    We use the geometry of a cylinder i.e., impose the open boundary condition 
    along the $y$-direction but the periodic boundary condition along the $x$-
    direction. This implies that the space is continuous along the $x$-direction 
    and any node very close to the $x=1$ line may have a right neighbor inside 
    the box and very close to the line $x=0$ and vice-versa.

    3. We agree. We add the following in the caption of Fig. 2(a):

    $N$ increases from top to bottom.
   
    4. Unfortunately due to our mistake the referee has misunderstood us. The
       critical value $\alpha_c$ of the parameter $\alpha$ is indeed -2. At a
       number of places including at the caption of the Fig. 2 we omitted the
       minus signs by mistake as pointed out by the first referee. We carefully 
       corrected them all. Therefore present range of $\alpha$ in Fig. 2(a) is 
       from -3 to 0 and covers well both sides of $\alpha_c$. We therefore keep 
       the Fig. 2 unchanged.

